Nuclear Mass Measurements With Radioactive Ion Beams

Nuclear masses are the most fundamental of all nuclear properties, yet they can provide a wealth of knowledge, including information on astrophysical sites, constraints on existing theory, and fundamental symmetries. In nearly all applications, it is necessary to measure nuclear masses with very high precision. As mass measurements push to more short-lived and more massive nuclei, the practical constraints on mass measurement techniques become more exacting. Various techniques used to measure nuclear masses, including their advantages and disadvantages are described. Descriptions of some of the world facilities at which the nuclear mass measurements are performed are given, and brief summaries of planned facilities are presented. Future directions are mentioned, and conclusions are presented which provide a possible outlook and emphasis on upcoming plans for nuclear mass measurements at existing facilities, those under construction, and those being planned.

==> introduction.tex <==
\section{Introduction}
Besides proof of particle stability, perhaps the most fundamental of nuclear properties is nuclear mass.  Knowledge of nuclear
masses can provide significant insight into other nuclear properties including, but not limited to, particle separation energies,
decay rates, shape, and shell model predictions.  Because of their intrinsic relationship to a host of other nuclear properties,
theoretical predictions and experimental determinations of nuclear masses have been a mainstay of nuclear research virtually since
its inception.  

Multiple techniques
for measuring nuclear mass have evolved over the years, each with characteristic advantages and disadvantages. In many cases,
the disadvantages of one particular technique are an advantage of another.  Applications of nuclear mass measurements to fundamental
nuclear physics and astrophysics will be discussed.  Mass measurement techniques will also be discussed along with the
facilities at which various methods are used.  Finally, future directions
in nuclear mass measurements will be presented.
\subsection{Applications of Nuclear Masses}
From an astrophysical standpoint, nuclear masses can provide
insight into properties of nucleosynthesis.  As an example,
the rapid neutron capture process - or \textit{r process} -
is thought to be responsible for production of roughly
half of all nuclei heavier than iron \cite{iliadis} and
nearly all of the actinides.  Because the r-process proceeds
via sequential neutron captures on existing nuclei, 
$^{A}$Z+n$\rightarrow^{A+1}$Z + $\gamma$, the
path of the r-process is strongly related to the 
mass of r-process progenitor nuclei.  The classical
r process path roughly follows a line of constant neutron
separation energy, $S_n$, where the neutron separation
energy is defined to be the amount of energy necessary
to remove a neutron from a nucleus, $S_n\equiv (M(Z,A) - M(Z,A-1))c^2$.
Knowledge of neutron separation energies is important
in understanding which nuclei are of particular importance
for the r-process.   In thermal equilibrium, the value of
$S_n$ depends on the environmental temperature.  For a
useful assessment of the properties of nuclei along the r
process path, the value of the neutron separation energy
should be known to within $kT\sim$100 keV, corresponding to
the temperature of the r-process environment.  


In other astrophysical applications, nuclear masses provide insight
into the thermodynamics of the environment.  Knowing the 
masses of nuclei involved in a reaction will allow for 
a calculation of the energy released in a reaction, which
can provide information on environmental heating.  Examples
where this might be important include neutron star crust heating \cite{meisel15,meisel16}, x-ray burst 
thermal properties \cite{rogers09}, stellar heating, and 
explosive nucleosynthesis.  
\subsection{Example: Nuclear Masses of Neutron-Rich Nuclei and the Astrophysical r Process}
\label{nucmasses}
The astrophysical r process is mentioned here as one example of an astrophysical site in which
nuclear mass measurements may be useful.  In the approximation of
(n,$\gamma$)$\rightleftharpoons$($\gamma$,n) equilibrium, corresponding to a 
the classical r process, nuclear masses can be used for 
a direct determination of neutron separation energies $S_n$.  
Though the canonical r-process may only have a limited contribution
to galactic abundances, nuclear masses are still useful for 
understanding shell structure far from stability \cite{pfeiffer01} for any
r-process scenario.  Minor shell closures, the disappearance of
shells, and the appearance of new shell structure can all inform theoretical 
development and evaluations of r-process sites.

Much of our current understanding of nuclei along the r-process path comes from extrapolating current
mass models to the r-process progenitor nuclei.  Of course, in the
absence of actually measuring r-process progenitor nuclei, pushing studies of nuclear properties to
more neutron-rich nuclei is advantageous.  Thus, there are compelling reasons to study
nuclei with increasing neutron richness as any extrapolation will then become more robust.  These studies may
be applicable to constraining mass models used in the r-process.

The impacts of nuclear mass uncertainties on an understanding of the r process have been studied in detail
in prior work \cite{martin16,mumpower15,atanasov15}.  Shell structure far from stability is important to
understand, but recent work has provided some interesting results which also indicate that 
the uncertainties in masses of the rare-earths must be constrained to better understand production
of these elements \cite{mumpower15,mumpower15b}.
\begin{figure}
	\vspace{-10pt}
	\includegraphics[width=1.0\linewidth,bb= 0 0 600 600,trim={4cm 4cm 4cm 4cm}]{meisel.pdf}
	\caption{Two-Neutron Separation energies for calcium nuclei (with the energy of the 2$^+$ yrast state indicated) for recent experimental
work \cite{meisel16} compared to various evaluations.  Used with permission \cite{meisel16}.}
	\label{s2nni}
	\vspace{-10pt}
\end{figure}

Mass models used to determine S$_n$ for
neutron-rich nuclei can disagree significantly.  Some
mass models predict smooth trends in S$_n$ along isotopic lines while others may predict shifts in the slope of S$_n$ as nuclei move further from stability, correlating with nuclear shape changes.  Regions of ``shape coexistence'' may exist in the table of isotopes where nuclei along isotopic lines go from being prolate to oblate (or vice versa).  Of course, different models result in different astrophysical results in various scenarios. 

As an example of the importance of mass measurements, consider Figure~\ref{s2nni}, which shows S$_{2n}$ trends along the Ca isotopic chain for 
experimental work compared to various theoretical models.  The differences become more pronounced with neutron richness.  This is not 
surprising as models can only be compared to and optimized with known masses. Mass measurements are necessary to constrain models for more exotic nuclei. 
Along isotopic chains, even measuring masses that are one nucleon beyond known masses can provide significant constraints on existing models.

Good overviews of nuclear data needs for astrophysical applications can 
also be found in Refs. \cite{kajino19,sun15,matos09}, and \cite{rahaman08}.
